Greedy Morse matchings and discrete smoothness

Discrete Morse theory emerged as an essential tool for computational geometry and topology. Its core structures are discrete gradient fields, defined as acyclic matchings on a complex $C$, from which topological and geometrical informations of $C$ can be efficiently computed, in particular its homology or Morse-Smale decomposition. Given a function $f$ sampled on $C$, it is possible to derive a discrete gradient that mimics the dynamics of $f$. Many such constructions are based on some variant of a greedy pairing of adjacent cells, given an appropriate weighting. However, proving that the dynamics of $f$ is correctly captured by this process is usually intricate. This work introduces the notion of discrete smoothness of the pair $(f,C)$, as a minimal sampling condition to ensure that the discrete gradient is geometrically faithful to $f$. More precisely, a discrete gradient construction from a function $f$ on a polyhedron complex $C$ of any dimension is studied, leading to theoretical guarantees prior to the discrete smoothness assumption. Those results are then extended and completed for the smooth case. As an application, a purely combinatorial proof that all CAT(0) cube complexes are collapsible is given.

==> other_text.tex <==

end of the cap 3 not used in the article

\subsection{Computational Examples}

Again, we would like to highlight that the focus of the work was theoretical. Our results for this chapter have been shown throughout the previous sections through the lemmas and theorems and are valid for any dimension. We decided to leave the list of tasks to implement what is a problem with the matching in question.

With the well-defined algorithm and proven geometric guarantees, our next step is to see the almost greedy matching applied in practice. The results are very similar to the results of Chapter~\ref {weddings}. Given our geometric assurances that compare the greedy matching with the almost greedy matching, this is not a surprise. In some cases, the resulting discrete gradients will differ in terms of noise and the number of unsaturated critical simplexes.

As in the previous chapter, the computational examples were realized through planar triangulations (simplistic complexes of dimension $2$) in grid form.

O primeiro resultado é mostrado na Figura~\ref{ruido_cancelado}. Nele retomamos o exemplo que motiva a noção de ruido no gradiente. Do lado esquerdo temos o gradiente discreto produzido pelo casamento guloso enquanto que do lado direito temos o gradiente discreto produzido pelo casamento quase guloso. A função avaliada nos vértices da triangulação é $f(x,y)=-x^2-y^2$ e novamente o domínio é dado por $x=[-2,2]$ e $y=[-2,2]$. 

The first result is shown in Figure~\ref{cancel-noise}. In it we return to the example that motivates the notion of noise in the gradient. On the left side we have the discrete gradient produced by the greedy matching while on the right side we have the discrete gradient produced by almost greedy matching. The function evaluated at the vertices of triangulation is $f(x,y)=-x^2-y^2$ and again the domain is given by $x=[-2,2]$ and $y=[-2,2]$. 

IMAGEM

Still in Figure ~\ref{chancelled noise}, note that the almost greedy matching did not produce the noise present in the discrete gradient built by greedy matching. This type of result suggests that, as we implement the new algorithm, it acts in a way to soften the discrete gradient; after all, it eliminates discrete gradient noise.

Thinking in this sense, we decided to disrupt the function in order to induce errors in the weight of its evaluated vertices. We would like to test whether the almost greedy matching can remove discrete gradient noise from inaccurate input data. For example, consider $f(x,y)=arctan(xy)$ in the domain $x=[-2,2]$ and $y=[- 2,2]$ evaluated at the vertices of a planar triangulation and its respective discrete gradient associated with greedy matching or almost greedy matching (Figure~\ref{atanxy_limpo}).

IMAGEM

Now consider the function $f(x,y)=arctan(xy)+\epsilon$ where $\epsilon \sim N(0,0.12)$ includes an error according to the normal distribution \footnote{After including $\epsilon$ in the last sum, $f$, would formally be considered a distribution.} with the same domain $x=[-2,2]$ e $y=[-2,2]$. The discrete gradient constructed through the greedy and almost greedy marriage is shown through Figure~\ref{atanxy_apagando_roido}~(a) and Figure~\ref{atanxy_apagando_roido}~(b), respectively.

IMAGEM

While in the first case we had a total of $6$ discrete gradient noise identified, in the second we had only $2$.

This latter practical result motivates that in fact the almost greedy matching can reduce noise in the discrete gradient from input data with errors. However, in Figure~\ref{atanxy_apagando_ruido}~(b) and comparing it with Figure~\ref{atanxy_limpo}, we still have $2$  present gradient noises - in addition to other undesirable critical simplexes that we did not address in this dissertation. This suggests that our algorithm is not able to capture and reduce all noise in the discrete gradient.

Thinking about this, during the research we decided to propose changes to the almost greedy matching seeking to improve it in the sense of trying to reduce all noise in the discrete gradient.

\section{Improvements to Almost Sweet Wedding}

In some cases, occurrences of discrete gradient noise still persist even using almost greedy matching.
In fact, this was expected. What we deal with since the beginning of the chapter was a structure that would potentially generate noise in the discrete gradient. Our condition checked, before selecting a minimum edge to be matched, whether it consisted of the central edge of a tree of $3$ width. But is the matching of this central edge the only way for the algorithm to generate noise in the discrete gradient ($3$ size-augmenting path)?

Figure~\ref{g_00} shows an example of construction in which we will still have noise in the discrete gradient even without having produced a tree of $3$ width in the process. More than that, this last figure suggests other structures that potentially generate close unsaturated vertices. Note that the $0$ weight edge will be matched by the almost greedy algorithm and will produce augmentation path.

IMAGEM

Thinking about what was said, we extended the algorithm almost greedy making its condition of when not match more "loose." This is done through a small modification: instead of verifying that an edge constitutes a central edge of a tree of width $3$, it is sufficient (in some aspects) to check if the neighboring vertices of one of the edges of the edge that will be selected have equal degree to $1$.

The results of this new almost greedy matching algorithm were very promising in order to reduce even more discrete gradient noise. The next figure illustrates an example. On the left side we have the construction of the discrete gradient from the greedy matching and from the right side from this new algorithm mentioned. The function used is still $f(x,y)=arctan(xy)+\epsilon$ where $\epsilon \sim N(0,0.12)$ with domain $ x = [- 2,2] $ e $ y = [-2.2]$. Look at Figure ~ \ ref {atanxy_apagando_mega_roido}.
 
IMAGEM

In this example, all $6$ discrete gradient noises were eliminated (in contrast to the $4$ noise eliminated by the almost greedy marriage). Not only, several undesirable critical (which do not represent the function) were also eliminated.

We will not include theoretical guarantees of this algorithm because, in addition to being complex, they do not guarantee part of the geometric guarantees that the other algorithms mentioned in the dissertation assure - such as the matter of decay (Theorems ~ \ ref {backsight}}, ~ \ ref {backsight_q}) or of the comparison between greedy and almost greedy matching (Theorema ~ \ ref {dif_estruturas}). Even so, we have decided to quote you as a guideline for future work.

We believe that the greedy algorithm can incorporate conditions that will make it a method to construct softer discrete gradients. From the way we implement it, it is clear to realize that we can extend reasoning and try to attack incremental paths with sizes larger than $3$, and thus seek to eliminate more critical critical similes. We also indicate that such a proposal must be calibrated in order to avoid the elimination of critical simplexes that actually represent the function in the discretized object. We intend, therefore, to generalize this notion soon.

